Multi-resolution Enhancement for Full Spectrum Neural Representations

Scientific data acquisition continues to outpace storage and analysis capabilities, making voxel-based representations increasingly intractable. Implicit neural representations (INRs) offer a promising solution by encoding signals through coordinate-based neural networks, serving as surrogates of data, with computational and storage requirements scaling with network complexity rather than data dimensionality. However, smaller INRs struggle to faithfully represent the multi-scale structures, high-frequency information, and fine textures that constitute a large proportion of scientific measurements. We propose WIEN-INR, a theoretically-guided hierarchical INR framework that distributes modeling across resolution scales and enables improved representation capacity through a novel enhancement network to recover subtle details. This multi-scale architecture allows smaller networks to retain the full spectrum of information while preserving training efficiency and lowering storage cost. Evaluated on distinct raw experimental measurements across scales and complexities, WIEN-INR represents a practical step toward broader adoption of neural representations in scientific workflows, delivering compact, robust, and high-fidelity representations.

==> Table/Cu3Au_data_table.tex <==
\begin{tabular}{rlrrrr}
\toprule
\small
Compression Rate & Method & PSNR (dB) & Time Taken (s) & Model Size (Bytes) & Compression Rate \\
\midrule
0.000500 & MLP (No Encoding) & 36.539160 & 13.203361 & 15152.000000 & 0.000348 \\
0.000500 & MLP (Freq Encoding) & 36.562106 & 13.129076 & 16816.000000 & 0.000386 \\
0.000500 & SIREN (No Encoding) & 36.692784 & 18.698508 & 20664.000000 & 0.000474 \\
0.000500 & WIRE (No Encoding) & 36.424712 & 37.965319 & 21064.000000 & 0.000484 \\
0.000500 & TCNN (No Encoding + ReLu) & 25.264850 & 32.994855 & 40960.000000 & 0.000940 \\
0.000500 & Wavelet-INR & 36.986939 & 14.747540 & 146088.000000 & 0.003354 \\
0.000500 & Wavelet-INR+ & 37.454786 & 28.712309 & 167976.000000 & 0.003856 \\
0.001000 & MLP (No Encoding) & 36.528138 & 16.781234 & 30102.000000 & 0.000691 \\
0.001000 & MLP (Freq Encoding) & 36.633982 & 16.595532 & 32566.000000 & 0.000748 \\
0.001000 & SIREN (No Encoding) & 36.709479 & 24.809104 & 42114.000000 & 0.000967 \\
0.001000 & WIRE (No Encoding) & 36.602963 & 60.460330 & 41656.000000 & 0.000956 \\
0.001000 & TCNN (No Encoding + ReLu) & 32.367627 & 31.211134 & 45056.000000 & 0.001034 \\
0.001000 & Wavelet-INR & 37.253494 & 14.599881 & 161712.000000 & 0.003712 \\
0.001000 & Wavelet-INR+ & 37.604479 & 30.821914 & 169578.000000 & 0.003893 \\
0.002000 & MLP (No Encoding) & 36.599934 & 19.764874 & 60414.000000 & 0.001387 \\
0.002000 & MLP (Freq Encoding) & 36.669451 & 20.139449 & 64030.000000 & 0.001470 \\
0.002000 & SIREN (No Encoding) & 36.721751 & 30.872292 & 86178.000000 & 0.001978 \\
0.002000 & WIRE (No Encoding) & 36.617202 & 79.514627 & 85504.000000 & 0.001963 \\
0.002000 & TCNN (No Encoding + ReLu) & 36.812565 & 31.576794 & 100352.000000 & 0.002304 \\
0.002000 & Wavelet-INR & 37.797573 & 15.886924 & 196968.000000 & 0.004522 \\
0.002000 & Wavelet-INR+ & 38.164406 & 31.315337 & 189378.000000 & 0.004348 \\
0.004000 & MLP (No Encoding) & 36.643022 & 32.062343 & 121104.000000 & 0.002780 \\
0.004000 & MLP (Freq Encoding) & 36.696205 & 32.980343 & 126352.000000 & 0.002901 \\
0.004000 & SIREN (No Encoding) & 36.728019 & 51.087759 & 175224.000000 & 0.004023 \\
0.004000 & WIRE (No Encoding) & 36.669827 & 134.581627 & 176296.000000 & 0.004047 \\
0.004000 & TCNN (No Encoding + ReLu) & 36.893704 & 30.761587 & 158208.000000 & 0.003632 \\
0.004000 & Wavelet-INR & 38.952686 & 17.478676 & 279216.000000 & 0.006410 \\
0.004000 & Wavelet-INR+ & 39.897054 & 34.044994 & 270186.000000 & 0.006203 \\
0.008000 & MLP (No Encoding) & 36.655328 & 44.270804 & 238284.000000 & 0.005470 \\
0.008000 & MLP (Freq Encoding) & 36.715202 & 44.381838 & 245772.000000 & 0.005642 \\
0.008000 & SIREN (No Encoding) & 36.750617 & 72.448035 & 348264.000000 & 0.007995 \\
0.008000 & WIRE (No Encoding) & 36.669424 & 233.297426 & 349756.000000 & 0.008029 \\
0.008000 & TCNN (No Encoding + ReLu) & 36.987253 & 30.960690 & 266880.000000 & 0.006127 \\
0.008000 & Wavelet-INR & 40.557124 & 19.748985 & 453096.000000 & 0.010402 \\
0.008000 & Wavelet-INR+ & 41.659328 & 40.998166 & 439116.000000 & 0.010081 \\
0.015000 & MLP (No Encoding) & 36.660924 & 75.137835 & 446544.000000 & 0.010251 \\
0.015000 & MLP (Freq Encoding) & 36.723154 & 74.713424 & 456912.000000 & 0.010489 \\
0.015000 & SIREN (No Encoding) & 36.801202 & 118.439479 & 657144.000000 & 0.015086 \\
0.015000 & WIRE (No Encoding) & 36.699935 & 360.020329 & 659176.000000 & 0.015133 \\
0.015000 & TCNN (No Encoding + ReLu) & 37.058737 & 31.506117 & 470464.000000 & 0.010800 \\
0.015000 & Wavelet-INR & 41.452607 & 23.414310 & 763056.000000 & 0.017517 \\
0.015000 & Wavelet-INR+ & 42.623630 & 51.479010 & 738924.000000 & 0.016963 \\
0.030000 & MLP (No Encoding) & 36.691808 & 121.906549 & 903102.000000 & 0.020732 \\
0.030000 & MLP (Freq Encoding) & 36.723983 & 121.940846 & 917982.000000 & 0.021074 \\
0.030000 & SIREN (No Encoding) & 37.389904 & 195.331881 & 1336482.000000 & 0.030681 \\
0.030000 & WIRE (No Encoding) & 36.676835 & 571.742714 & 1333696.000000 & 0.030617 \\
0.030000 & TCNN (No Encoding + ReLu) & 37.118472 & 32.739404 & 850688.000000 & 0.019529 \\
0.030000 & Wavelet-INR & 42.334379 & 32.742820 & 1427112.000000 & 0.032762 \\
0.030000 & Wavelet-INR+ & 43.566555 & 71.390489 & 1390500.000000 & 0.031921 \\
0.050000 & MLP (No Encoding) & 36.630603 & 174.843754 & 1351058.000000 & 0.031016 \\
0.050000 & MLP (Freq Encoding) & 36.727276 & 174.876284 & 1369330.000000 & 0.031435 \\
0.050000 & SIREN (No Encoding) & 37.154690 & 277.478120 & 2004282.000000 & 0.046012 \\
0.050000 & WIRE (No Encoding) & 36.653046 & 769.351459 & 2000860.000000 & 0.045933 \\
0.050000 & TCNN (No Encoding + ReLu) & 37.315892 & 33.391758 & 2870336.000000 & 0.065894 \\
0.050000 & Wavelet-INR & 42.770289 & 41.327087 & 2276136.000000 & 0.052253 \\
0.050000 & Wavelet-INR+ & 44.275076 & 99.802080 & 2271912.000000 & 0.052156 \\
0.070000 & MLP (No Encoding) & 36.633685 & 200.922316 & 1598612.000000 & 0.036699 \\
0.070000 & MLP (Freq Encoding) & 36.738918 & 201.026051 & 1618516.000000 & 0.037156 \\
0.070000 & SIREN (No Encoding) & 39.148131 & 317.531714 & 2373624.000000 & 0.054491 \\
0.070000 & WIRE (No Encoding) & 36.772682 & 892.662847 & 2377444.000000 & 0.054579 \\
0.070000 & TCNN (No Encoding + ReLu) & 37.419190 & 31.816172 & 9506112.000000 & 0.218230 \\
0.070000 & Wavelet-INR & 43.085913 & 51.833626 & 3194856.000000 & 0.073344 \\
0.070000 & Wavelet-INR+ & 44.693380 & 118.745921 & 3136020.000000 & 0.071993 \\
0.150000 & MLP (No Encoding) & 36.625222 & 700.832030 & 4710722.000000 & 0.108143 \\
0.150000 & MLP (Freq Encoding) & 36.745910 & 697.669521 & 4745122.000000 & 0.108933 \\
0.150000 & SIREN (No Encoding) & 40.735945 & 1079.706674 & 7024122.000000 & 0.161252 \\
0.150000 & WIRE (No Encoding) & 36.759345 & 2080.021909 & 7017676.000000 & 0.161104 \\
0.150000 & TCNN (No Encoding + ReLu) & 37.453827 & 34.776411 & 17148992.000000 & 0.393687 \\
0.150000 & Wavelet-INR & 43.932079 & 82.611746 & 6666408.000000 & 0.153040 \\
0.150000 & Wavelet-INR+ & 37.852955 & 202.599082 & 6062694.000000 & 0.139180 \\
\bottomrule
\end{tabular}


==> Table/XCS.tex <==
\begin{table}[]
    \centering
\resizebox{\textwidth}{!}{
    \begin{tabular}{rlrrrr}
        \toprule
        Hidden Features & Method & PSNR (dB) & Time Taken (s) & Model Size (Bytes) & Compression Rate \\
        \midrule
124 & MLP (No Encoding) & 36.603 & 20.790 & 143488 & 0.003 \\
124 & MLP (Freq Encoding) & 36.679 & 20.901 & 151424 & 0.003 \\
124 & SIREN (No Encoding) & 36.704 & 32.501 & 205488 & 0.005 \\
124 & WIRE (No Encoding) & 36.672 & 86.556 & 207152 & 0.005 \\
124 & TCNN (No Encoding + Sin) & 36.979 & 8.791 & 2870336 & 0.066 \\
124 & Wavelet (New Method) & 38.352 & 17.940 & 210348 & 0.005 \\
160 & MLP (No Encoding) & 36.653 & 30.436 & 231184 & 0.005 \\
160 & MLP (Freq Encoding) & 36.684 & 29.565 & 241424 & 0.006 \\
160 & SIREN (No Encoding) & 36.737 & 47.538 & 334224 & 0.008 \\
160 & WIRE (No Encoding) & 36.691 & 130.370 & 336320 & 0.008 \\
160 & TCNN (No Encoding + Sin) & 37.380 & 9.190 & 54263104 & 1.246 \\
160 & Wavelet (New Method) & 39.234 & 18.495 & 325440 & 0.007 \\
196 & MLP (No Encoding) & 36.657 & 42.122 & 339616 & 0.008 \\
196 & MLP (Freq Encoding) & 36.704 & 42.070 & 352160 & 0.008 \\
196 & SIREN (No Encoding) & 36.766 & 65.569 & 494064 & 0.011 \\
196 & WIRE (No Encoding) & 36.674 & 168.211 & 496592 & 0.011 \\
196 & TCNN (No Encoding + Sin) & 37.422 & 22.643 & 408133376 & 9.369 \\
196 & Wavelet (New Method) & 40.143 & 19.356 & 463824 & 0.011 \\
232 & MLP (No Encoding) & 36.630 & 44.504 & 468784 & 0.011 \\
232 & MLP (Freq Encoding) & 36.697 & 44.629 & 483632 & 0.011 \\
232 & SIREN (No Encoding) & 36.790 & 70.519 & 685008 & 0.016 \\
232 & WIRE (No Encoding) & 36.674 & 231.741 & 687968 & 0.016 \\
232 & TCNN (No Encoding + Sin) & 37.420 & 34.058 & 707028352 & 16.231 \\
232 & Wavelet (New Method) & 40.764 & 20.417 & 625920 & 0.014 \\
268 & MLP (No Encoding) & 36.657 & 55.605 & 618688 & 0.014 \\
268 & MLP (Freq Encoding) & 36.711 & 54.537 & 635840 & 0.015 \\
268 & SIREN (No Encoding) & 36.725 & 87.745 & 907056 & 0.021 \\
268 & WIRE (No Encoding) & 36.697 & 278.089 & 910448 & 0.021 \\
268 & TCNN (No Encoding + Sin) & 15.016 & 9.283 & 37120 & 0.001 \\
268 & Wavelet (New Method) & 41.414 & 23.462 & 812556 & 0.019 \\
304 & MLP (No Encoding) & 36.660 & 63.453 & 789328 & 0.018 \\
304 & MLP (Freq Encoding) & 36.724 & 63.429 & 808784 & 0.019 \\
304 & SIREN (No Encoding) & 36.823 & 101.257 & 1160208 & 0.027 \\
304 & WIRE (No Encoding) & 36.730 & 316.503 & 1164032 & 0.027 \\
304 & TCNN (No Encoding + Sin) & 16.092 & 7.510 & 45056 & 0.001 \\
304 & Wavelet (New Method) & 41.464 & 24.319 & 1022172 & 0.023 \\
340 & MLP (No Encoding) & 36.653 & 76.305 & 980704 & 0.023 \\
340 & MLP (Freq Encoding) & 36.712 & 76.579 & 1002464 & 0.023 \\
340 & SIREN (No Encoding) & 36.801 & 121.213 & 1444464 & 0.033 \\
340 & WIRE (No Encoding) & 36.718 & 378.682 & 1448720 & 0.033 \\
340 & TCNN (No Encoding + Sin) & 36.577 & 8.165 & 158208 & 0.004 \\
340 & Wavelet (New Method) & 41.702 & 26.559 & 1256544 & 0.029 \\
376 & MLP (No Encoding) & 36.639 & 81.748 & 1192816 & 0.027 \\
376 & MLP (Freq Encoding) & 36.721 & 81.777 & 1216880 & 0.028 \\
376 & SIREN (No Encoding) & 37.184 & 130.675 & 1759824 & 0.040 \\
376 & WIRE (No Encoding) & 36.731 & 412.032 & 1764512 & 0.041 \\
376 & TCNN (No Encoding + Sin) & 36.988 & 7.782 & 2870336 & 0.066 \\
376 & Wavelet (New Method) & 41.817 & 27.968 & 1513680 & 0.035 \\
412 & MLP (No Encoding) & 36.685 & 104.969 & 1425664 & 0.033 \\
412 & MLP (Freq Encoding) & 36.726 & 104.601 & 1452032 & 0.033 \\
412 & SIREN (No Encoding) & 36.756 & 166.506 & 2106288 & 0.048 \\
412 & WIRE (No Encoding) & 36.729 & 481.103 & 2111408 & 0.048 \\
412 & TCNN (No Encoding + Sin) & 37.231 & 8.839 & 30670400 & 0.704 \\
412 & Wavelet (New Method) & 41.949 & 30.758 & 1795788 & 0.041 \\
448 & MLP (No Encoding) & 36.680 & 116.623 & 1679248 & 0.039 \\
448 & MLP (Freq Encoding) & 36.731 & 116.747 & 1707920 & 0.039 \\
448 & SIREN (No Encoding) & 37.203 & 185.720 & 2483856 & 0.057 \\
448 & WIRE (No Encoding) & 36.690 & 510.899 & 2489408 & 0.057 \\
448 & TCNN (No Encoding + Sin) & 37.405 & 22.703 & 408133376 & 9.369 \\
448 & Wavelet (New Method) & 42.226 & 31.411 & 2100444 & 0.048 \\
484 & MLP (No Encoding) & 36.549 & 127.921 & 1953568 & 0.045 \\
484 & MLP (Freq Encoding) & 36.715 & 127.944 & 1984544 & 0.046 \\
484 & SIREN (No Encoding) & 36.894 & 203.849 & 2892528 & 0.066 \\
484 & WIRE (No Encoding) & 36.685 & 626.485 & 2898512 & 0.067 \\
484 & TCNN (No Encoding + Sin) & 37.401 & 34.442 & 707028352 & 16.231 \\
484 & Wavelet (New Method) & 42.291 & 35.241 & 2430288 & 0.056 \\
        \bottomrule
        \end{tabular}
    }
    \caption{XCS Results Table}
    \label{tab:XCS}
\end{table}


==> Table/camera_super4x_table.tex <==
\begin{table}[]
    \centering
\resizebox{\textwidth}{!}{
\begin{tabular}{rlrrrr}
\toprule
Hidden Features & Method & PSNR (dB) & Time Taken (s) & Model Size (Bytes) & Compression Rate \\
\midrule
64 & MLP (No Encoding) & 19.066 & 10.213 & 34308 & 0.033 \\
64 & MLP (Freq Encoding) & 22.080 & 10.184 & 38404 & 0.037 \\
64 & SIREN (No Encoding) & 31.416 & 15.324 & 50948 & 0.049 \\
64 & WIRE (No Encoding) & 28.092 & 30.567 & 51752 & 0.049 \\
64 & Wavelet (New Method) & 33.510 & 14.623 & 205352 & 0.196 \\
88 & MLP (No Encoding) & 20.034 & 12.135 & 64068 & 0.061 \\
88 & MLP (Freq Encoding) & 22.883 & 12.141 & 69700 & 0.066 \\
88 & SIREN (No Encoding) & 33.047 & 18.801 & 95396 & 0.091 \\
88 & WIRE (No Encoding) & 27.912 & 48.741 & 96488 & 0.092 \\
88 & Wavelet (New Method) & 37.315 & 14.636 & 339272 & 0.324 \\
112 & MLP (No Encoding) & 20.435 & 14.020 & 103044 & 0.098 \\
112 & MLP (Freq Encoding) & 23.634 & 14.182 & 110212 & 0.105 \\
112 & SIREN (No Encoding) & 34.352 & 22.402 & 153668 & 0.147 \\
112 & WIRE (No Encoding) & 27.524 & 56.470 & 155048 & 0.148 \\
112 & Wavelet (New Method) & 40.550 & 15.986 & 514664 & 0.491 \\
136 & MLP (No Encoding) & 20.888 & 19.236 & 151236 & 0.144 \\
136 & MLP (Freq Encoding) & 23.864 & 19.026 & 159940 & 0.153 \\
136 & SIREN (No Encoding) & 35.919 & 30.693 & 225764 & 0.215 \\
136 & WIRE (No Encoding) & 31.085 & 87.036 & 227432 & 0.217 \\
136 & Wavelet (New Method) & 42.645 & 18.325 & 731528 & 0.698 \\
\bottomrule
\end{tabular}
}
\end{table}

==> ref.tex <==
Lu, Y., Jiang, K., Levine, J., \& Berger, M. (2021). Compressive Neural Representations of Volumetric Scalar Fields. Computer Graphics Forum, 40. https://doi.org/10.1111/cgf.14295

Lee, S., Jeong, J., \& Ryu, E. (2023). Entropy-Constrained Implicit Neural Representations for Deep Image Compression. IEEE Signal Processing Letters, 30, 663-667. https://doi.org/10.1109/LSP.2023.3279780

Han, J., Zheng, H., & Bi, C. (2023). KD-INR: Time-Varying Volumetric Data Compression via Knowledge Distillation-Based Implicit Neural Representation. IEEE Transactions on Visualization and Computer Graphics, 30, 6826-6838. https://doi.org/10.1109/TVCG.2023.3345373

Li, H., & Zhang, X. (2024). Human–Machine Collaborative Image Compression Method Based on Implicit Neural Representations. IEEE Journal on Emerging and Selected Topics in Circuits and Systems, 14, 198-208. https://doi.org/10.1109/JETCAS.2024.3386639

Pistilli, F., Valsesia, D., Fracastoro, G., & Magli, E. (2022). Signal Compression via Neural Implicit Representations. ICASSP 2022 - 2022 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP), 3733-3737. https://doi.org/10.1109/icassp43922.2022.9747208

Dupont, E., Goli'nski, A., Alizadeh, M., Teh, Y., & Doucet, A. (2021). COIN: COmpression with Implicit Neural representations. ArXiv, abs/2103.03123. 

Strümpler, Y., Postels, J., Yang, R., Gool, L., \& Tombari, F. (2021). Implicit Neural Representations for Image Compression. **, 74-91. https://doi.org/10.1007/978-3-031-19809-0_5

Schwarz, J., Tack, J., Teh, Y., Lee, J., \& Shin, J. (2023). Modality-Agnostic Variational Compression of Implicit Neural Representations. ArXiv, abs/2301.09479. https://doi.org/10.48550/arXiv.2301.09479

Strümpler, Y., Postels, J., Yang, R., Gool, L., & Tombari, F. (2021). Implicit Neural Representations for Image Compression. , 74-91. https://doi.org/10.1007/978-3-031-19809-0_5.


